Deciphering the Underserved: Benchmarking LLM OCR for Low-Resource Scripts

This study investigates the potential of Large Language Models (LLMs), particularly GPT-4o, for Optical Character Recognition (OCR) in low-resource scripts such as Urdu, Albanian, and Tajik, with English serving as a benchmark. Using a meticulously curated dataset of 2,520 images incorporating controlled variations in text length, font size, background color, and blur, the research simulates diverse real-world challenges. Results emphasize the limitations of zero-shot LLM-based OCR, particularly for linguistically complex scripts, highlighting the need for annotated datasets and fine-tuned models. This work underscores the urgency of addressing accessibility gaps in text digitization, paving the way for inclusive and robust OCR solutions for underserved languages.

==> sections/motivation.tex <==
\section{Motivation}

Low-resource languages such as Urdu, Albanian, and Tajik, with their complex structural features—bidirectional text, diacritic variations, and modified Cyrillic alphabets—pose significant challenges for traditional OCR systems, which rely on static datasets and heuristic methods. In contrast, Large Language Models (LLMs) offer a dynamic, context-aware alternative, but their effectiveness for OCR in such scripts under varied conditions remains largely unexplored. By systematically benchmarking LLM performance on these underserved languages, alongside English as a control, this study seeks to reveal their potential for robust digitization, addressing key gaps in accessibility and digital preservation for linguistically diverse communities.

